MTRGL:Effective Temporal Correlation Discerning through Multi-modal Temporal Relational Graph Learning

In this study, we explore the synergy of deep learning and financial market applications, focusing on pair trading. This market-neutral strategy is integral to quantitative finance and is apt for advanced deep-learning techniques. A pivotal challenge in pair trading is discerning temporal correlations among entities, necessitating the integration of diverse data modalities. Addressing this, we introduce a novel framework, Multi-modal Temporal Relation Graph Learning (MTRGL). MTRGL combines time series data and discrete features into a temporal graph and employs a memory-based temporal graph neural network. This approach reframes temporal correlation identification as a temporal graph link prediction task, which has shown empirical success. Our experiments on real-world datasets confirm the superior performance of MTRGL, emphasizing its promise in refining automated pair trading strategies.

==> tex/preliminary.tex <==
\section{Preliminaries}

Let $\mathcal{A} = \{A_1, A_2, ..., A_n\}$ be a set of $n$  entities (e.g., companies, assets or markets) under consideration. Each $A_i$ is characterized by a two tuple $A_i := (X_i, P_i(t))$.  $X_i = (x^{(1)}, x^{(2)}, ..., x^{(m)})$ is a feature vector, where each entries $x^{(j)}$ represents the the $j$-th features of entity $A_i$. (e.g., name of the sector, trading volume, market share, e.t.c.).  $P_i(t): t \mapsto \mathbb{R}$ is the time series of the trading price of entity $A_i$. 

As discussed earlier, convergent trading is a strategy that exploits temporary price inefficiencies, expecting that the price will 'converge' to a fair value or a mean over time. 
One common form of convergent trading is pairs trading, where traders take a long position in one entity and a short position in a related entity when their prices diverge in a way that is statistically anomalous. Traders aim to profit when the prices 'converge' back to their historical relationship. Therefore, we can interpret that the goal of convergence (pair) trading is to identify pair of entities $A_i$ and $A_j$ whose prices have a strong correlation. Suppose the price of $A_i$ rises while the price of $A_j$ remains the same, causing a divergence in their historical correlation. In response, the trader sell short an amount of $A_i$ (betting that its price will fall) and buy an equal amount of $A_j$ (betting that its price will rise).  If the prices of $A_i$ and $A_j$ return to their historical correlation, the trader can close both positions for a profit.

